Functional principal component analysis for global sensitivity analysis of model with spatial output

Motivated by risk assessment of coastal flooding, we consider time-consuming simulators with a spatial output. The aim is to perform sensitivity analysis (SA), quantifying the influence of input parameters on the output. There are three main issues. First, due to computational time, standard SA techniques cannot be directly applied on the simulator. Second, the output is infinite dimensional, or at least high dimensional if the output is discretized. Third, the spatial output is non-stationary and exhibits strong local variations. We show that all these issues can be addressed all together by using functional PCA (FPCA). We first specify a functional basis, such as wavelets or B-splines, designed to handle local variations. Secondly, we select the most influential basis terms, either with an energy criterion after basis orthonormalization, or directly on the original basis with a penalized regression approach. Then FPCA further reduces dimension by doing PCA on the most influential basis coefficients, with an ad-hoc metric. Finally, fast-to-evaluate metamodels are built on the few selected principal components. They provide a proxy on which SA can be done. As a by-product, we obtain analytical formulas for variance-based sensitivity indices, generalizing known formula assuming orthonormality of basis functions.

==> SubFiles/results.tex <==
\subsection{Comparison of GP-PCA and GP-FPCA}
We consider the same notations introduced in section \ref{kriging_FPCA}.

\subsubsection{Wavelet decomposition}

The type of wavelets and the level of decomposition is chosen according to the decomposition error. For one type of decomposition, we decompose the 500 output maps for different level of decomposition. We compute the local mean square errors (RMSE) of decomposition: 

%\begin{equation}
%RMSE_{wavelet}(z) = \sqrt{\frac{1}{n}\sum_{i=1}^n(y_{x^{(i)}}(z)-\tilde{y}_{x^{(i)}}(z))^2]}
%\end{equation}

\begin{equation}
MSE_{wavelet}(z) = \frac{1}{n}\sum_{i=1}^n(y_{x^{(i)}}(z)-\tilde{y}_{x^{(i)}}(z))^2]
\end{equation}  

with $\tilde{y}$ is the map approximated by wavelet decomposition. Then, we observe the spatial mean of $MSE_{decompo}(z)$. 

%\begin{equation}
%RMSE_{wavelet} = \sum_{k=1}^{nr=194}\sum_{l=1}^{nc=202} RMSE_{wavelet}(z_{k,l})
%\end{equation}

\begin{equation}
MSE_{wavelet} = \sum_{k=1}^{nr=194}\sum_{l=1}^{nc=202} MSE_{wavelet}(z_{k,l})
\end{equation}

\begin{figure}[H]
\begin{center}
\includegraphics[scale=0.5]{MseWaveletDecomposition}
\end{center}
\caption{$RMSE_{wavelet}$ for different type of wavelets (which are included on the R package "waveslim") and level of decomposition, from 1 to 6.}
\label{error_decompo}
\end{figure}

We choose the type and the level of decomposition where $MSE_{wavelet}$ is minimised. Therefore, we decompose the maps using the Daubechies wavelet of moment $4$ ("d4") with $1$ level of decomposition. In fact, figure \ref{error_decompo} shows that the lower values of MSE is reached for "d4", and constant values between $1$ and $6$ levels of decomposition.

\subsubsection{PCA on the most informative wavelet coefficients}

To predict the map, we have to determine the proportion of spatial energy $p$ (which implies the number of wavelet of coefficient ) and the number of principal components $n_{PC}$ such as the error of prediction is minimised at most. To study the efficiency of GP-FPCA , we use the $10$-fold cross-validation method. The sample of $500$ simulations is splited onto $10$ sub-samples (then sub-samples with $50$ observations). The outputs one of them are assumed to be unknown, and are predicted by GP-FPCA based on the $9$ other sub-samples. The process is repeated for each sub-sample. For different values of $p$ and $n_{PC}$, wa compute the spatial RMSE of the functional model for each sub-sample.

\begin{equation}
RMSE(z) = \sqrt{\mathbb{E}_{\mathbf{X}}\left[(y_{\mathbf{X}}(z) - \hat{y}_{\mathbf{X}}(z))^2 \right] }
\label{rmse}
\end{equation}

Then, we make the mean of the RMSE of all sub-samples. The calibration of $p$ and $n_{PC}$ has made according to the spatial mean of (\ref{rmse}).

\begin{figure}[H]
\begin{center}
\includegraphics[scale=0.8]{\PathS calibration_FPCA_BRGM}
\caption{Calibration of $p$ and $n_{PC}$ for GP-FPCA. $p\in\left\{0.7;0.8;0.9;0.95;0.98;0.99\right\}$  and $n_{PC}\in \left\{1,\dots,10\right\}$}
\label{calibration}
\end{center}

\end{figure}     

The mean RMSE \JR{is} minimised for $p=0.99$ (in average $3492$ wavelet coefficients), and \JR{converges for} $n_{PC}=2$ (in average, $95.6\%$ of the explained variance). Therefore, we choose these values for the model.

\subsubsection{Prediction efficiency of GP-PCA vs GP-FPCA} 

In the following, we centred $Y_\mathbf{X}$: $\mathbb{E}_{\mathbf{X}}[y_\mathbf{X}(z)]=0$. In the figures, the empty area corresponds $0$ cm of water level. 
 
\begin{figure}[H]
\begin{center}
\includegraphics[width = 0.3\textwidth]{\PathS RMSE_FPCA_nPC2_p99}
\includegraphics[width=0.3\textwidth]{\PathS RMSE_PCA_nPC2}
\includegraphics[width=0.3\textwidth]{\PathS diff_methods}
\caption{From left to right, the RMSE map for GP-FPCA, the one for GP-PCA, and the absolute value of the difference between both of them.}
\end{center}
\end{figure}
 
The RMSE of GP-FPCA is more uniform over the space than GP-PCA. In fact, by using wavelet basis, PCA \JR{does the projection of} the output map area by area, \JR{instead} of \JR{"qu'entends-tu par traditional?"}traditional method which projected it point by point independently. Furthermore, the global map varies between $0$cm and $20$cm of error. For GP-PCA, the RMSE is not uniform over the space. We even see two areas : yellow area and red area. The RMSE of the yellow area is from $0$cm to $15$cm lower than GP-FPCA. In the red area, the RMSE is higher from $20$cm to $40$cm than GP-FPCA. This area corresponds to the zone where there are most of the discontinuities, which could not take into account by projecting point by point as for traditional PCA. The error on the area, where GP-FPCA is less accurate, is much less important that the one where GP-PCA is. Therefore, GP-FPCA is more accurate than GP-PCA. Furthermore, with 3 cores \JRC{DONNER ICI le détail du PROCESSEUR UTILISE, e.g. with a XXX GHz quadri-core processor and XXX GB of RAM}, GP-FPCA is six times faster than GP-PCA. The saving time is not proportional to the number of modelling wavelet coefficients, because of the computation time of wavelet decomposition.\\    

\subsection{Global Sensitivity Analysis}

% ICI je propose une reformulation; desole ai fait une fausse manip et ai efface qqs bouts.

\JR{First, we analyse the principal components derived from the FPCA of the 500 simulated flooding maps (step 4 of the procedure), see figure (\ref{PC}.}

\begin{figure}[H]
\includegraphics[width = 0.45\textwidth]{\PathS First_PC}
\includegraphics[width=0.45\textwidth]{\PathS Second_PC}
\caption{Principal Components (PC) of the $500$ simulated maps. Right, first PC ($86.6\%$ of the explained variance). Left, second PC ($9\%$ of the explained variance). Total proportion of variance of both PC: $95.6\%$. }
\label{PC}
\end{figure}

\JRC{Puisque tu parles de la moyenne des cartes, il faudrait donner l'image}.
\JR{Figure \ref{PC} provides the two firs PCs that represent $95.6\%$ of the total variation (that corresponds to a satisfactory level of explained variance). Note that we centered the output model, level $0$} (empty area) corresponds to the mean over space of water level. Colors from yellow to red are positive values, and show the average increase of water level (from $0$cm to more than $2$cm with respect to the spatial mean). Those from green to blue are negative, and show the average decrease of water level (from $0$cm to $4$cm with respect to the spatial mean). The first PC corresponds to the increase of water level on the whole map, especially in the red area where are the highest growth of the water level (up to more than $2$cm). The second PC shows highest increase of water level in the same area of the yellow one of the first PC, and decrease of water level in the green and blue area.\\

\JR{The  estimate of the Sobol indices are then evaluated using a Monte-Carlo-based approach. These estimates require several thousands of model runs (see e.g., \cite{saltelli2008global}), and to overcome the computational burden of this task, we use the GP-FPCA model (set up in Sect.} \JRC{"RENVOYER A LA SECTION CORRESPONDANTE"}\JR{) to replace the expensive-to-evaluate numerical simulator.
The global sensitivity analysis is performed on each principal component, and to derive the synthetic criterion, we apply equation }\JRC{"RENVOYER A LA SECTION CORRESPONDANTE"}. \JR{This allows to highlight the inputs which influence the most spatial distribution of the flooding-induced water height.}


%two first order indices and two total indices for each principal components. 
%Finally, to get the synthetic criterion, we have made the mean of them, weighted by the associated eigenvalues. In this way, we synthesize the influence of each input of $95.6\%$ of the total variation, which corresponded to the proportion of explained variance of the two first PC. This proportion has considered enough for the study. 

% J'ai pas compris cette phrase
\JRC{"J'ai pas compris cette phrase:"First, the GP-FPCA model error converge from $n_{PC}=2$. If the $4.4\%$ explained variance has considered, it can also lead to over-learning.}\\          

%\begin{figure}[H]
%\begin{center}
%\includegraphics[scale=0.5]{\PathS curve_sensi}
%\caption{Sensitivity Analysis Overview}
%\end{center}
%\end{figure}


\begin{figure}[H]
\begin{center}
\includegraphics[scale=0.5]{\PathS GSI_FPCA}
\caption{Spatial \JR{Sobol indices. Top: first order et total order indices. Bottom: second order indices}. \JRC{#### Sur cette figure, changer le nom des variables en cohérence avec le texte (phi-> to, t1-> t-, etc., changer le titre des figures (c'est en français)}}
\label{spatialSI}
\end{center}
\end{figure}
% JR: proposition de reformulation:
\JR{Figure \ref{spatialSI} provides the spatial distribution of the Sobol indices (first order and total indices - top and interaction terms- bottom) calculated with the algorithm of} \JRC{"A RENSEIGNER" with "A RENSEIGNER"} \JR{Monte-Carlo random simulations. The interpretation is similar to the Sobol indices for scalar outputs. The analysis of the main effects show that the individual contributions of the parameters taken alone only contribute to a small part to the whole variability; $T$ has the largest contribution to the variance of about $10\%$. The analysis of the total effects Figure \ref{spatialSI}(top) is more informative and shows that the major contributors are $T$ and $to$ (with total indices of the same order of magnitude of about 0.70) followed by $S$, $t_{-}$ and $t_{+}$ with total indices of the order of 0.20-0.40. A deeper analysis of the second order Sobol indices (Figure \ref{spatialSI}, bottom) shows that it is the interaction of $T$ and $t_o$ that drives the most the variability.} 
%The figure 7 represents the spatial sobol indices. Their interpretation is same as traditional sobol indices. Among all the indices, the total set themselves apart, especially $T$ and $t_0$, which influenced the output between $60\%$ and $80\%$. On the contrary, their respective first order indices show that they only have less than $10\%$ of influence by themselves (without interactions with other inputs). Nevertheless, the total indices of $S$, $t_{-}$ and $t_{+}$ are $20\%$, and $30\%$ for the two last inputs, which were not negligible. By themselves, they have any influence according to their associated first order indices. //   

